Learning Low-dimensional Latent Dynamics from High-dimensional Observations: Non-asymptotics and Lower Bounds

In this paper, we focus on learning a linear time-invariant (LTI) model with low-dimensional latent variables but high-dimensional observations. We provide an algorithm that recovers the high-dimensional features, i.e. column space of the observer, embeds the data into low dimensions and learns the low-dimensional model parameters. Our algorithm enjoys a sample complexity guarantee of order $\tilde{\mathcal{O}}(n/\epsilon^2)$, where $n$ is the observation dimension. We further establish a fundamental lower bound indicating this complexity bound is optimal up to logarithmic factors and dimension-independent constants. We show that this inevitable linear factor of $n$ is due to the learning error of the observer's column space in the presence of high-dimensional noises. Extending our results, we consider a meta-learning problem inspired by various real-world applications, where the observer column space can be collectively learned from datasets of multiple LTI systems. An end-to-end algorithm is then proposed, facilitating learning LTI systems from a meta-dataset which breaks the sample complexity lower bound in certain scenarios.

==> sections/a1_relatedwork.tex <==
\section{Related Literature}
\label{app:lit-rev}
\paragraph{Other Linear Models with Low-Dimensional Dynamics. } 
Recently, there are lines of research on autoregressive models with low-dimensional representations \cite{dong_extracting_2022, poloni_closed-form_2019, qin_latent_2022}. Indeed, we may also be able to reconstruct low-dimensional dynamics from the model with the learned representations. However, sample complexity results are not currently available for such models. Another related line of research is on dynamic factor models \cite{breitung_dynamic_2006, anderson_linear_2022, hallin_factor_2023}. \citet{anderson_linear_2022} only provides asymptotic convergence guarantees. Finite time convergence is indeed developed in \citet{hallin_factor_2023}. However, their results can not imply dependence on the system dimensions and are only about the error decaying rates. Moreover, certain assumptions might not be easily verified in our setting. 

\paragraph{General SYSID Algorithms. } The most relevant sample complexity results are provided in recent literature including but not restricted to \citet{oymak_non-asymptotic_2019,sarkar_finite_2021,zheng_non-asymptotic_2021}. The former two papers focus on system with stable latent dynamics, while the last paper extends to unstable latent dynamics. Unfortunately, all algorithms have sample complexity $\calO(n\text{poly}(r)/\epsilon^2)$, which not only depends on $n$ but also has polynomial factors on $r$. 
There also exist a line of work providing sample complexities for systems without observers \cite{sarkar_near_2019, shirani_faradonbeh_finite_2018}, whose analysis techniques is applicable to unstable dynamics. 
This paper focuses on stable latent dynamics, and we put into future directions to extend the results to unstable scenarios. 

\paragraph{Existing SYSID Lower Bounds. } There exist literature providing lower bounds for SYSID in our setting. However, their results are not directly comparable to ours in our setting. The most relevant papers are \citet{sun_finite_2023, fattahi_learning_2021}. The former provides a lower bound depending on $r/n$, which is tailored for systems with $r \gg n$. The latter provides a lower bound proportional to $1/\epsilon^4$, which follows a slower rate than ours, though being logarithmic in the system dimensions. \citet{sun_finite_2022} provides lower bounds defined for noise-free settings. \citet{mao_finite-time_2021} provides lower bounds for systems with $C = I$. \citet{bakshi_new_2023} provides lower bounds for learning almost uncontrollable and unobservable systems. Other related works include \citet{djehiche_non_2021, jedra_finite-time_2023, simchowitz_learning_2018}, which develop lower bound for systems without observers. 

\paragraph{General Subspace Learning Algorithms. } To learn the observer column space, several existing techniques may be applicable. \citet{balzano_streaming_2018, candes_robust_2011, vaswani_robust_2018, blanchard_statistical_2007} focus on analysis for PCA subspace learning. However, they assume the data distribution to be i.i.d., which is not the case for dynamic systems. Dynamic factor model techniques are also applicable \cite{hallin_factor_2023}. As discussed previously, the results can not imply the dependence on the system dimensions. Some other ideas include \citet{deng_invariant_2020}, whose sample complexity remains open. 


\section{Additional Notations}
Let $\kl(\bbQ||\bbP) \coloneqq \bbE_{\bbQ}\b{\log\frac{\d \bbQ}{\d \bbP}}$ be the KL-divergence of two distributions $\bbP, \bbQ$.
Let $e_i$ be the one-hot vector with $1$ in the $i$-th coordinate and let $E_{i,j}$ be the matrix with a $1$ in the $(i,j)$-th coordinate and zeros elsewhere. For matrix A, define $\Gamma_t(A) = \sum_{\tau=0}^{t}A^\tau (A^\tau)\t$. 

